Aerobat, A Bioinspired Drone to Test High-DOF Actuation and Embodied Aerial Locomotion

This work presents an actuation framework for a bioinspired flapping drone called Aerobat. This drone, capable of producing dynamically versatile wing conformations, possesses 14 body joints and is tail-less. Therefore, in our robot, unlike mainstream flapping wing designs that are open-loop stable and have no pronounced morphing characteristics, the actuation, and closed-loop feedback design can pose significant challenges. We propose a framework based on integrating mechanical intelligence and control. In this design framework, small adjustments led by several tiny low-power actuators called primers can yield significant flight control roles owing to the robot's computational structures. Since they are incredibly lightweight, the system can host the primers in large numbers. In this work, we aim to show the feasibility of joint's motion regulation in Aerobat's untethered flights.

==> unused.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/aerobat_ks_joint_id.pdf}
    \caption{The linkage model of the Aerobat's KS which consists of 7 linkages and 10 joints, labeled $L_i$ and $J_j$, respectively. $J_1$, $J_5$, and $J_8$ positions are fixed on the body while $L_1$ represents the gear/crank moment arm. The angle of joint $i$ ($\theta_i$) is defined with respect to the body's $y$-axis, e.g. shown in this image is the angle of joint 5 ($\theta_5$).}
    \label{fig:ks_linkages_details}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/linkages_length.pdf}
    \caption{Linkage dimensions of the Aerobat's KS mechanism. There are 16 linkage parameters and 6 joint positions ($J_1$, $J_5$, and $J_8$) which determine the resulting flapping trajectory.}
    \label{fig:aerobat_linkages_dimensions}
\end{figure}



\begin{table}[t]
    %\vspace{0.1in}
    \centering
    \caption{Sensitivity Analysis of the Armwing KS Parameters}
    %\vspace{-0.1in}
    \begin{tabular}{c | c c c c c}
    \toprule
    $\bm{q}$ & $A_s$ & $A_e$ & $M_s$ & $M_e$ & $\Delta \theta$ \\
    \midrule
    $l_1$    & 200   & 205   & -9.00 & -124  & 4.32$\cdot 10^{3}$ \\
    $l_{2a}$ & 6.97  & -137  & -204  &  244  & -1.54$\cdot 10^{3}$ \\
    $l_{2b}$ & 0     & 183   & 0     & -306  & 0 \\
    $l_{2c}$ & 0     & 115   & 0     & -193  & 0 \\
    $l_{3a}$ & 0     & -1.81 & 0     &  22.3 & -2.26$\cdot 10^{3}$ \\
    $l_{3b}$ & -124  & -67.9 & -65.8 & 119   & 1.06$\cdot 10^{4}$ \\
    $l_{3c}$ & -111  & 148   & 90.2  & -263  & 0 \\
    $\alpha_3$ & 0   & 1.26  & 1.00  & -2.11 & 0 \\
    $l_{4}$  & 0     & 220   & 0     & -367  & 1.56$\cdot 10^{4}$ \\
    $l_{5a}$ & 0     & -68.5 & 0     & -20.4 & -1.33$\cdot 10^{4}$ \\
    $l_{5b}$ & 0     & -217  & 0     & 356   & -8.88$\cdot 10^{3}$ \\
    $l_{5c}$ & 0     &  3.11 & 0     & -8.70 & -1.43$\cdot 10^{3}$ \\
    $l_{5d}$ & 0     & -22.3 & 0     &  48.4 &  0 \\
    $l_{6}$  & 0     &  22.5 & 0     & -49.2 &  0 \\
    $l_{7b}$ & 0     & -28.7 & 0     &  42.9 &  0 \\
    $l_{7c}$ & 0     & -12.2 &  0    & -10.1 &  0\\
    $p_{1y}$ & 7.50  & -11.2 & -158  & 69.0  &  3.24$\cdot 10^{3}$\\
    $p_{1z}$ & 4.78  &  131  & -123  & -189  &  7.59$\cdot 10^{3}$\\
    $p_{5y}$ & -7.04 &  157  &  159  & -203  &  -6.97$\cdot 10^{2}$\\
    $p_{5z}$ & -4.83 &  78.1 &  123  & -190  &  0\\
    $p_{8y}$ & 0     & -147  &  0    &  135  &  -1.55$\cdot 10^{3}$\\
    $p_{8z}$ & 0     & -208  &  0    &  378  &  -1.09$\cdot 10^{4}$\\
    \bottomrule
    \multicolumn{6}{l}{Note: units are rad/m or rad/rad (for $\alpha_3$). \Tstrut}
    \end{tabular}
    %\vspace{-0.1in}
    \label{tab:sensitivity}
\end{table}


\begin{table}[t]
    %\vspace{0.1in}
    \centering
    \caption{Sensitivity Analysis of the Wing Mechanism Parameters}
    %\vspace{-0.1in}
    \begin{tabular}{c | c c c c c}
    \toprule
    $\bm{q}$ & $A_s$ & $A_e$ & $M_s$ & $M_e$ & $\Delta \theta$ \\
    \midrule
    $l_1$ & \textbf{19.7} &\textbf{ 47.7} & -1.40 & -3.47 & \textbf{18.6} \\
    $l_2$ & -2.79 & 2.48 & 9.86 & -28.6 &  -4.71 \\
    $l_{3a}$ & -2.94 & -17.7 & -10.2 &  30.9 & -1.23 \\
    $l_{3b}$ &  -1.51 &  8.85 & 11.1 & \textbf{-30.97} & -5.21 \\
    $l_{3c}$ &  1.87 & 2.93 & -2.06 & 5.74 & 0 \\
    $l_4$ &   1.83 & -8.14 & \textbf{-11.3} &  31.6 & 3.81 \\
    $l_{5a}$ & -5.49 &  -19.8 &   -6.83 &  22.5  & -5.37 \\
    $l_{5b}$ & -7.47 &  -6.59 &   7.79 & -21.5 &  -7.89 \\
    $\alpha_5$ & 0  & 68.5  & 57.3 & -163 & 0 \\
    $p_{4y}$ & -6.96 &  -6.22 &   8.56 & -21.4226 & -12.4 \\
    $p_{7x}$ & -2.36 &   7.40 &  11.0 & -30.3708 &  -6.19 \\
    $p_{7y}$ &  4.22 &  11.3  &  1.28 &  -9.05 &  5.18 \\
    $\phi_{0}$ &  -2.2$\cdot 10^{-4}$ & -2.3$\cdot 10^{-4}$ & -4.3$\cdot 10^{-4}$ & -2.5$\cdot 10^{-4}$ & 0 \\
    $l_6$ & 0 &  \textbf{-23.7} & 0&  14.2 &  \textbf{-20.8} \\
    $l_7$ & 0 &   8.69 &  0 &  \textbf{-24.9} &    1.5\\
    $l_{8a}$ & 0 &   12.3 &  0 &  -15.0 &    5.4\\
    $l_{8b}$ & 0 &   -9.5 &  0 &   15.0 &  -5.14\\
    $l_{8c}$ & 0 &  -1.14 &  0 &  -14.0 &   -5.4\\
    $l_9$ & 0 &    6.07 &  0 &  -20.9 &   -2.0\\
    $l_{10a}$ &  0 &    10.8 &  0 &  -16.5 &    7.2\\
    $l_{10b}$ &  0 &    4.36 &  0 &   11.7 &   7.71\\
    $l_{10c}$ &  0 &   -2.37 &  0 &  0.045 &  0.514\\
    $l_{10d}$ &  0 &   -1.08 &  0 &    2.5 &      0\\
    $l_{11}$ &  0 &    1.01 &  0 &  -2.77 &      0\\
    $l_{12a}$ &  0 &    -1.3 &  0 &   2.51 &      0\\
    $l_{12b}$ &  0 &  -0.434 &  0 &  -1.08 &      0\\
    $p_{12y}$ & 0 &   -6.09 &  0 &   10.6 &   -3.6\\
    $p_{14x}$ & 0 &   -6.51 &  0 &   15.5 &   2.28\\
    $p_{14y}$ & 0 &   -4.28 &  0 &   16.3 &      0\\
    $\Delta \phi$ & 0 &   117.0 &  0 &   12.1 &      0\\
    \bottomrule
    \multicolumn{6}{l}{Note: units are rad/mm for length or position and rad/rad for angles. \Tstrut}
    \end{tabular}
    %\vspace{-0.1in}
    \label{tab:sensitivity}
\end{table}
